Multivariate Confidence Calibration for Object Detection

Unbiased confidence estimates of neural networks are crucial especially for safety-critical applications. Many methods have been developed to calibrate biased confidence estimates. Though there is a variety of methods for classification, the field of object detection has not been addressed yet. Therefore, we present a novel framework to measure and calibrate biased (or miscalibrated) confidence estimates of object detection methods. The main difference to related work in the field of classifier calibration is that we also use additional information of the regression output of an object detector for calibration. Our approach allows, for the first time, to obtain calibrated confidence estimates with respect to image location and box scale. In addition, we propose a new measure to evaluate miscalibration of object detectors. Finally, we show that our developed methods outperform state-of-the-art calibration models for the task of object detection and provides reliable confidence estimates across different locations and scales.

==> chapter/definitions.tex <==
\section{Definitions}
\label{section:definitions}
Let the input $\inputvariate \in \inputset$, the class label $\classvariate \in \classset = \{1 , ... \numclasses\}$ and all box information $\numvariates$ given by $\bboxvariate_1 \in \bboxset_1$, ..., $\bboxvariate_\numvariates \in \bboxset_\numvariates$  denote random variates that follow a joint ground truth distribution $\priormodel(\inputvariate, \classvariate, \bboxvariate_1, ..., \bboxvariate_\numvariates) = \priormodel(\classvariate, \bboxvariate_1, ..., \bboxvariate_\numvariates | \inputvariate) \priormodel(\inputvariate)$. We further denote $\allbboxvariates = \{\bboxvariate_1, ..., \bboxvariate_\numvariates\}$ as all ground truth box information available. A detection model $\model$ is interpreted as a probabilistic model $\estimatedmodel(\classvariate, \allbboxvariates | \inputvariate)$ that outputs class predictions $\predclassvariate \in \classset$ with a confidence $\predvariate$ and the corresponding box proposals $\predbboxvariate_1 \in \bboxset_1$, ..., $\predbboxvariate_\numvariates \in \bboxset_\numvariates$  as the regression outcome. This is further denoted as $\allpredbboxvariates = \{\predbboxvariate_1, ..., \predbboxvariate_\numvariates\}$ as all propsed box information, so that $\model(\inputvariate) = (\predclassvariate, \predvariate, \allpredbboxvariates)$. Furtermore, let $\matchedvariate \in \matchedset = \{0, 1\}$ denote if a prediction of the model $\model(\inputvariate)$ has matched the ground truth box with the right class at a certain Intersection of Union (IoU) score. 

By definition, an object detection model is perfectly calibrated if 
\begin{align}
\label{eq:calibration}
& \underbrace{\prob(\matchedvariate=1 | \predvariate = \probscore, \predclassvariate = \class, \predbboxvariate_\indexvariates = \bbox_\indexvariates)}_{\text{accuracy given } \probscore, \class, \bbox_\indexvariates} = \underbrace{\probscore}_{\text{confidence}}, \\ \nonumber
& \forall \probscore \in [0,1], \class \in \classset, \bbox_\indexvariates \in \bboxset_\indexvariates, \indexvariates \in \{1..\numvariates\}
\end{align}
is fulfilled. On classification tasks, this is usually not achievable by any known method \cite{Guo2018}. We assume this statement for detection tasks as well.
In contrast to classification, measuring the miscalibration of a detection model also depends on the IoU score used to determine if a box proposal $\allpredbboxes \in \allpredbboxvariates$ matches a ground truth box $\allbboxes \in \allbboxvariates$.

By using the indicator if the ground truth box has matched or not, we break down all calibration tasks to simple binary calibration.
Let $\calmodel$ denote a model that outputs a calibrated confidence estimate in a post processing step. On classification, this model only needs the class prediction and the according confidence estimate. However, we investigate if additional box information are needed for object detection calibration. Thus, we define a calibration model for object detection by $\calmodel(\classvariate, \predvariate, \allpredbboxvariates)$. We further denote a single confidence estimate as $\confidence$ and the according calibrated score as $\calibrated$.

Typical box information are the box center coordinates \centerx, \centery and the width/height \width, \height. We can use these box information relative to the image size. This restricts the space of the random variates $\allbboxvariates$ to the interval 
\begin{align}
\bboxset_\indexvariates \in [0, 1], \quad \forall \indexvariates \in 1 .. \numvariates.
\end{align}
Thus, we do not need to distinguish between the confidence estimates and the predicted box information any more as we treat all available information as random variates in the interval $[0, 1]$. Therefore, if we assume an own calibration model for each class defined in $\classset$, we can define $\collectvariate = \{\predvariate, \predbboxvariate_1, ..., \predbboxvariate_\numvariates\}$ as the collection of all predicted information by a model $\model$ with a single outcome $\collect$.

For our further investigations, we assume $\numclasses = 1$ as an object detection task for a single class. By using separate models for different classes, all calibration methods for object detection might also be extended to multi-class.

